LWeb: Information Flow Security for Multi-tier Web Applications

This paper presents LWeb, a framework for enforcing label-based, information flow policies in database-using web applications. In a nutshell, LWeb marries the LIO Haskell IFC enforcement library with the Yesod web programming framework. The implementation has two parts. First, we extract the core of LIO into a monad transformer (LMonad) and then apply it to Yesod's core monad. Second, we extend Yesod's table definition DSL and query functionality to permit defining and enforcing label-based policies on tables and enforcing them during query processing. LWeb's policy language is expressive, permitting dynamic per-table and per-row policies. We formalize the essence of LWeb in the $\lambda_{LWeb}$ calculus and mechanize the proof of noninterference in Liquid Haskell. This mechanization constitutes the first metatheoretic proof carried out in Liquid Haskell. We also used LWeb to build a substantial web site hosting the Build it, Break it, Fix it security-oriented programming contest. The site involves 40 data tables and sophisticated policies. Compared to manually checking security policies, LWeb imposes a modest runtime overhead of between 2% to 21%. It reduces the trusted code base from the whole application to just 1% of the application code, and 21% of the code overall (when counting LWeb too).

==> labeled.tex <==
\section{Labeled Values}\label{sec:labeled}

==> labelling.tex <==
\section{Manipulation of Labeled Values}\label{sec:labeling}
In~\S~\ref{sec:labels} we provide the primitive @TLabeled@ to 
generate labeled values. 
To enforce noninterference, we offered 
% But, for noninterference, we had 
no way to unlabel such values. 
%
Now that we have monadic operations that propagate the current label, 
% , and after we used the monadic operations to propagate the current label, 
we extend the terms of our programs to allow for explicit 
manipulation of labeled values. 

\paragraph{Terms}
The term @TTLabel tl t@ labels the term @t@
with the label term @tl@. 
The term @TUnlabel t@ returns the value of the labeled term @t@, 
while term @TLabelOf t@ returns @t@'s label.   
\begin{mcode}
  data Term l = ...  
    | TTLabel  (Term l) (Term l) 
    | TUnlabel (Term l) 
    | TLabelOf (Term l)
\end{mcode}

\paragraph{Values} All of the introduced terms are evaluated, thus are not values. 
\begin{mcode}
  isValue (TTLabel _ _) = False   
  isValue (TUnlabel _)  = False  
  isValue (TLabelOf _)  = False
\end{mcode}

\paragraph{Term Evaluation}
We extend term evaluation to evaluate the @TLabelOf t@ term.
\begin{mcode}
  evalTerm (TLabelOf (TLabeled l _)) 
    = TLabel l 
  evalTerm (TLabelOf t)
    = TLabelOf (evalTerm t) 
\end{mcode}
If the argument @t@ is evaluated to the @TLabeled l _@ value, 
then evaluation returns the label @l@, otherwise the argument @t@ is evaluated. 
Note that if @t@ is evaluated to a different value, then 
the evaluation will get stuck repeating the evaluation of a non-labeled value. 
%
To catch such errors, we can use an type system 
that separates labeled expressions from the rest. 
% We can use a type system to catch such errors, but 
% 
This error does not affect the noninterference proof since 
our proof assumes terminating programs.


\paragraph{Program Evaluation}
Labeling and unlabeling expressions are monadic terms
since they 
depend on 
%require reading and writing \resp
the label state. 

The term @TTLabel tl t@ labels the term @t@
with the label @tl@. 
First the term @tl@ is evaluated into a label @l@. 
If the current program label can flow into @l@, 
then the monadic labeled value @TLabeled l t@
is returned. 
Otherwise, a runtime exception is thrown. 
\begin{mcode}
  eval (Pg lc (TTLabel (TLabel l) t))
    | lc canFlowTo l 
    = Pg lc (TReturn (TLabeled l t))
    | otherwise 
    = Pg lc TException
  eval (Pg lc (TTLabel tl t))
    = Pg lc (TTLabel (evalTerm tl) t)
\end{mcode}

The term @TUnlabel t@ unlabels the term @t@. 
First the term @t@ is evaluated into a 
labeled value @TLabeled l t@. 
Then, term @t@ is returned 
while the current label is raised to the join of the 
old label and @l@.
\begin{mcode}
  eval (Pg lc (TUnlabel (TLabeled l t)))
    = Pg (l join lc) (TReturn t)
  eval (Pg lc (TUnlabel t))
    = Pg lc (TUnlabel (evalTerm t))
\end{mcode}


\paragraph{Erasure}
Program erasure remains the same.
Term erasure is updated to aggressively
erase terms @t@ that are about to get labeled with a label @l1@
that does not flow to @l@. \NV{Can we skip that erasing and still have noninterference?}
For the rest of the terms, erasure is a homomorphism.
\begin{mcode}
  εTerm l (TTLabel (TLabel l1) t)  
    | l1 canFlowTo l 
    = TTLabel (TLabel l1) (εTerm l t)
    | otherwise
    = TTLabel (TLabel l1) THole 
  εTerm l (TTLabel tl t)  
    = TTLabel (εTerm l tl) (εTerm l t)
  εTerm l (TUnlabel t)   = TUnlabel (εTerm l t)
  εTerm l (TLabelOf t)   = TLabelOf (εTerm l t)
\end{mcode}

\paragraph{Noninterference}
To prove noninterference under the extended expressions, 
we update the simulations proof for programs and expressions. 

Our extensions break the simulations proof of~\S~\ref{subsection:lio:noninterference}
for the case that the current program label cannot flow into the erasure label.
This is not surprising, since unlabeling is the first term 
whose evaluation modifies the current label.
Thus, after this extension, 
the evaluation of the program @Pg lc t@ can return with a different label, say @lc'@. 
In the modification of the proof (below), 
we use monotonicity of labels during evaluation and the transitivity of 
@(canFlowTo)@ to show that if the erasure of the program  @Pg lc t@ reduces to a hole
then so does the evaluation @eval (Pg lc t)@.
\begin{mcode}
  simulations l (Pg lc t) 
    | not (lc canFlowTo l) 
    =   ε l (eval (ε l (Pg lc t)))
    ==. ε l (eval PgHole)
    ==. ε l PgHole
    ==. PgHole
    ==. ε l (Pg lc' t')
        ? monotonicEval (Pg lc t) &&& 
          lawFlowTransitivity lc lc' l 
    ==. ε l (eval (Pg lc t)) 
    *** QED 
    where (Pg lc' t') = eval (Pg lc t)
\end{mcode}
%

For each new monadic expression, we need to add a case in the 
simulations proof. 
Most of the cases are proven 
by following the cases splitting of evaluation and erasure. 
Interestingly, since erasure can happen before or after evaluation,
@TTLabel tl t@  requires the distinction of three cases 
for the term @tl@:
1) @tl@ is a label
2) @tl@ is not a label, but evaluates in one step in a label (thus erasure happens after evaluation) 
3) none of the above, thus erasure does not happen.
\NV{not sure if this makes sense... check again}
\JP{I'd say either add more detail/example or drop this}
 


==> labels.tex <==
\section{Labels in Terms}\label{sec:labels}

\subsection{Security Lattice}

\begin{figure*}

\begin{mcode}
  class Label l where
    (canFlowTo) :: l -> l -> Bool
    (meet) :: l -> l -> l
    (join) :: l -> l -> l

    lawFlowReflexivity  :: l:l  -> {l canFlowTo l}
    lawFlowAntisymmetry :: l1:l -> l2:l -> {(l1 canFlowTo l2 && l2 canFlowTo l1) => l1 == l2}
    lawFlowTransitivity :: l1:l -> l2:l -> l3:l -> { (l1 canFlowTo l2 && l2 canFlowTo l3) => l1 canFlowTo l3}

    lawMeet :: z:l -> l1:l -> l2:l -> l:l -> {z == l1 meet l2 <=> z canFlowTo l1 && z canFlowTo l2 && (l canFlowTo l1 && l canFlowTo l2 => l canFlowTo z)}
    lawJoin :: z:l -> l1:l -> l2:l -> l:l -> {z == l1 join l2 <=> l1 canFlowTo z && l2 canFlowTo z && (l1 canFlowTo l && l2 canFlowTo l => z canFlowTo l)}
\end{mcode}
\caption{Security Lattice as the Label type class}
\label{fig:label}
\end{figure*}

In figure~\ref{fig:label} we extend the @Label@ type class 
to define the security lattice of labels. 
%
The class contains three lattice methods: 
the ordering @(canFlowTo)@, pronounced ``can flow to'', 
the meet @(meet)@ and the join @(join)@.
The final five methods use refinement types to encode the class laws 
that must be satisfied. 

\paragraph{Partial Order}
If @l@ is a @Label@, then @(canFlowTo)@ defines a partial order on @l@. 
Thus, @(canFlowTo)@ should be reflexive, antisymmetric, and transitive, 
as respectively encoded by the refinements of the methods 
@lawFlowReflexivity@, @lawFlowAntisymmetry@, and @lawFlowTransitivity@. 
%
For instance, 
the call @lawFlowReflexivity l@ returns a proof (\ie a unit Haskell value)
that for all labels @l@, @l canFlowTo l@.
%
Moreover, to define an instance of the class @Label@, 
one needs to explicitly provide a reflexivity proof, as a class method. 


\paragraph{Lattice}
We refine the @lawMeet@ method to define the properties of the @(meet)@ lattice operator. 
Namely, for all labels @l1@ and @l2@, we define @z == l1 meet l2@ so that 
\begin{itemize}
\item @z@ can flow to @l1@ and @l2@ (@z canFlowTo l1 && z canFlowTo l2@)
\item all labels that can flow to @l1@ and @l2@, can also flow to @z@ 
@(forall l . l canFlowTo l1 && l canFlowTo l2 => l canFlowTo z)@.
\end{itemize}

Dually, we refine the @lawJoin@ method 
to describe @l1 join l2@ as the minimum label 
that is greater than @l1@ and @l2@. 

\paragraph{Using the label laws}
The label laws are class methods, which can be used for each @l@ that satisfies the 
@Label@ class constraints. 
%
For example below we prove that foreach labels @l1@, @l2@, and @l3@, 
if @l1@ cannot flow into @l3@, 
then @l1 join l2@ cannot flow into @l3@.
\begin{mcode}
  canNotFlowToJoin :: Label l => l1:l -> l2:l -> l3:l 
    -> { not (l1 canFlowTo l3) => not ((l1 join l2) canFlowTo l3) }
  canNotFlowToJoin l1 l2 l3 = 
    lawJoin (join l1 l2) l1 l2 l3  &&&
    lawFlowTransitivity l1 (join l1 l2) l3 
\end{mcode}
%
%
The proof proceeds by calling the laws of join and transitivity, 
while the contrapositive step is automatically enforced, 
since Liquid Haskell knows boolean logic. 

 
\subsection{Labels as Terms}
Our goal is to extend programs (of~\S~\ref{sec:non-interference}) 
to contain labels. 
Towards this goal, 
we define terms that manipulate labels. 
%
Terms consist of   
labels (@TLabel@), a labeled value (@TLabeled@) and 
label operations (@TOp@).
The labeled operations (@LabelOp@) 
are the binary operations of 
join, meet, or checking is a label flows to another. 
We also include the boolean terms @TTrue@ and @TFalse@
that will be the result of flow check. 
Finally, we include a hole term (@THole@)
that denotes erased terms (as explained in~\S~\ref{subsec:label:erasure}). 
\JP{This references a paragraph}

%
\begin{mcode}
  data Term l 
   = TLabel l
   | TOp LabelOp (Term l) (Term l) 
   | TLabeled l (Term l)
   | TTrue | TFalse 
   | THole 
   
data LabelOp = LMeet | LJoin | LCanFlowTo
\end{mcode}
%
Note that, the terms provide the labeled construct to label 
terms, but there is no construct to unlabel them.
Once a term is labeled there is no way to be accessed, 
which is crucial for proving noninterference. 

\paragraph{Values}
We distinguish values from terms that can get evaluated 
using the @isValue@ function. 
Up to now, only the label operation needs evaluation.
\begin{mcode}
  isValue :: Term l -> Bool 
  isValue TTrue          = True 
  isValue TFalse         = True 
  isValue (TLabel _)     = True 
  isValue (TLabeled _ _) = True 
  isValue THole          = True 
  isValue _              = False 
\end{mcode}

\paragraph{Evaluation}
We define term evaluation  
to evaluate the label operations and simply return values. 
%
To evaluate a label operation,  
first we fully evaluate the label arguments and then 
invoke the relevant @Label@ methods.  
%
\begin{mcode}
  evalTerm :: Label l => Term l -> Term l 
  evalTerm (TOp LMeet (TLabel l1) (TLabel l2)) 
    = TLabel (l1 meet l2) 
  evalTerm (TOp LJoin (TLabel l1) (TLabel l2)) 
    = TLabel (l1 join l2) 
  evalTerm (TOp LCanFlowTo (TLabel l1) (TLabel l2)) 
    = boolTerm (l1 canFlowTo l2) 
  evalTerm (TOp o (TLabel l1) t2)
    = TLOp o (TLabel l1) (evalTerm t2)
  evalTerm (TOp o t1 t2)
    = TLOp o (evalTerm t1) t2
  evalTerm v  | isValue v 
    = v     
\end{mcode}
%
When evaluating a meet or a join, 
the result is a label value
that gets converted into a term by the @TLabel@
constructor. 
%
When evaluating a @LCanFlowTo@ the result is a Haskell boolean 
that gets converted into a term using the @boolTerm@ function:
%
\begin{mcode}
  boolTerm :: Bool -> Term l 
  boolTerm True  = TTrue
  boolTerm False = TFalse 
\end{mcode}


\paragraph{Erasure}
We define the term erasure function 
to replace any term labeled with labels higher than the 
observation label with holes. 
\begin{mcode}
  εTerm :: Label l => l -> Term l -> Term l
  εTerm l (TLabeled l1 t) 
    | l1 canFlowTo l 
    = TLabeled l1 (εTerm l t)
    | otherwise 
    = TLabeled l1 THole
  εTerm l TTrue       = TTrue 
  εTerm l TFalse      = TFalse
  εTerm l (TLabel i)  = TLabel i
  εTerm l (TOp o x y) = TOp o (εTerm l x) (εTerm l y)
  εTerm l THole       = THole
\end{mcode}
When the erasure level is @l@,
all values labeled with labels that cannot flow to @l@
are replaced with holes. 
Otherwise, the erasure function is a homomorphism 
over terms. 

\subsection{Programs with Terms}
We extend programs to contain terms: 
\begin{mcode}
  data Program l 
    = PgHole 
    | Pg {pTerm :: Term l}
\end{mcode}
Now program evaluation, reduces to term evaluation. 
\begin{mcode}
  eval :: Label l => Program l -> Program l 
  eval PgHole = PgHole
  eval (Pg t) = Pg (evalTerm t)
\end{mcode}
Similarly, program erasure reduces to term erasure: 
\begin{mcode}
  ε :: Label l => l -> Program l -> Program l
  ε _ PgHole = PgHole
  ε l (Pg t) = Pg (εTerm l t) 
\end{mcode}
The nonintereference proof of~\S~\ref{sec:non-interference}
is still correct, since it relies on the simulations property 
of programs. 
But, the simulations property breaks, since 
erasure is no longer an identity. 
We conclude this section by proving the simulations property for 
our updated program definition. 


\subsection{Simulations}
We extend the simulations proof of~\S~\ref{subsec:non-interference:simulations}
to accommodate programs with terms.
%
\begin{mcode}
  simulations l (Pg t) 
    =   ε l (eval (ε l (Pg t)))
    ==. ε l (eval (Pg (εTerm l t)))
    ==. ε l (Pg (evalTerm (εTerm l t)))
    ==. Pg (εTerm l (evalTerm (εTerm l t)))
        ? simulationsTerm l t 
    ==. Pg (εTerm l (evalTerm t))   
    ==. ε l (Pg (evalTerm t))   
    ==. ε l (eval (Pg t))   
    *** QED
\end{mcode}
The proof proceeds by rewriting and 
is using the simulations property on terms.

\paragraph{Term Simulations}
Term simulation encodes the simulation between 
term evaluation @evalTerm@ and term evaluation after erasure
@evalTerm . εTerm l@. 
It is a property similar to the one expressed in Figure~\ref{fig:simulation}, 
but for terms instead of programs. 
\begin{mcode}
  simulationsTerm 
    :: Label l => l:l
    -> t:Term l
    -> { εTerm l (evalTerm (εTerm l t)) = εTerm l (evalTerm t) }
\end{mcode}
We prove the property by induction on the term input. 
The interesting case is where the term is labeled (@TLabeled l1 t@) 
since we need to case split on whether or not the term label @l1@
can flow into the erasing label @l@: 
% 
\begin{mcode} 
  simulationsTerm l (TLabeled l1 t)
    | l1 canFlowTo l 
    =   εTerm l (evalTerm (εTerm l (TLabeled l1 t))) 
    ==. εTerm l (evalTerm (TLabeled l1 (εTerm l t))) 
    ==. εTerm l (TLabeled l1 (εTerm l t)) 
    ==. TLabeled l1 (εTerm l (εTerm l t)) 
        ? εTermIdempotent l t 
    ==. TLabeled l1 (εTerm l t)
    ==. εTerm l (TLabeled l1 t)
    ==. εTerm l (evalTerm (TLabeled l1 t))
    *** QED  
    | otherwise 
    =   εTerm l (evalTerm (εTerm l (TLabeled l1 t))) 
    ==. εTerm l (evalTerm (TLabeled l1 THole)) 
    ==. εTerm l (TLabeled l1 THole) 
    ==. TLabeled l1 THole 
    ==. εTerm l (TLabeled l1 t)
    ==. εTerm l (evalTerm (TLabeled l1 t))
    *** QED  
\end{mcode}
If @l1 canFlowTo l@, 
then erasure of the term simply erases the term @t@
and the proof proceeds by rewriting and idempotence of erasure,
that is, erasing a term once is equivalent to erasing it twice. 
Otherwise, 
erasing a labeled term produces a hole, 
in which case the proof proceeds by rewriting. 


In the case of the label operation @TOp o t1 t2@, 
we split three cases, on whether or not the terms @t1@ and @t2@ are labels. 
\begin{mcode}
  simulationsTerm l (TOp o (TLabel l1) (TLabel l2))
    = ()
  simulationsTerm l (TOp o (TLabel l1) t2) 
    = simulations l t2
  simulationsTerm l (TOp o t1 t2)
    = simulations l t1 
\end{mcode}
When both terms are labels, the proof proceeds by rewriting
that is automatically performed by Liquid Haskell. 
When a term (say @t1@) is not a label, 
evaluation performs one step of evaluation on this term, thus
the proof requires an inductive call 
(say @simulations l t1@).

For the rest of the cases, both evaluation and erasure 
is an identity thus the proof is trivial.
\begin{mcode}
  simulationsTerm l t
    =   εTerm l (evalTerm (εTerm l t)) 
    ==. εTerm l (evalTerm t) 
    *** QED 
\end{mcode}

\paragraph{Idempotence}
\JP{Maybe we can move this to the appendix to save space.}
For completeness, we express and prove idempotence on term erasure.  
\begin{mcode}
  εTermIdempotent 
    :: Label l 
    => l:l 
    -> t:Term l 
    -> { εTerm l (εTerm l t) = εTerm l t } 

  εTermIdempotent l TTrue         
    = ()
  εTermIdempotent l TFalse        
    = ()
  εTermIdempotent l (TLabel _)    
    = ()
  εTermIdempotent l (TOp o t1 t2)  
    = εTermIdempotent l t1 &&& εTermIdempotent l t2 
  εTermIdempotent l (TLabeled l1 t) 
    | l1 canFlowTo l 
    = εTermIdempotent l t   
    | otherwise 
    = εTermIdempotent l t     
  εTermIdempotent l THole         
    = ()
\end{mcode}
The proof is performed by induction and case splitting 
following the definition of erasure.
In the label operations case,  
we use the infix proof combinator, @&&&@, % @x &&& _ = x@
to combine the two inductive proof terms. % into one.


==> lambda.tex <==
\section{Lambda Calculus Terms}\label{sec:lambda}

Next, we extend our terms to contain 
the standard lambda calculus primitives 
and discuss how the proof of simulations, and thus interference is preserved. 

\paragraph{Lambda Calculus Terms}
We extend the term definition to encode variables, 
application, lambda abstractions, and the fix combinator. 
%
\begin{mcode}
  type Var = Integer 

  data Term l = ...
    | TVar Var
    | TApp Term Term
    | TLam Var Term
    | TFix Term
\end{mcode}
%
In our proof we also encode 
commonly used terms like if, unit, and booleans,
but we omit them here for space. 

\paragraph{Values}
We extend the @isValue@ predicate
to denote the new terms that are not evaluated. 
\begin{mcode}
  isValue :: Term l -> Bool 
  isValue (TVar _)   = True 
  isValue (TLam _ _) = True 
  isValue _          = False 
\end{mcode}
\JP{Maybe drop for space}

\paragraph{Evaluation}
The function @evalTerm@ is extended with standard call-by-name
small step evaluation. 
%
\begin{mcode}
  evalTerm :: Term -> Term 
  evalTerm (TApp (TLam x t1) t2) 
    = subst x t2 t1 
  evalTerm (TApp t1 t2) 
    = TApp (evalTerm t1) t2 
  evalTerm (TFix (TLam x t)) 
    = subst x (TFix (TLam x t)) t
  evalTerm (TFix t) 
    = TFix (evalTerm t)

  subst :: Var -> Term -> Term -> Term
  ... 
\end{mcode}
@subst x tx t@ is naturally defined to 
recursively substitute @x@ with @tx@ in the term @t@.


\paragraph{Erasure}
Finally, we homomorphically extend term erasure 
over the new lambda calculus terms. 
\begin{mcode}
  εTerm :: Label l => l -> Term -> Term 
  εTerm _ (TVar x)   = TVar x 
  εTerm l (TApp f t) = TApp (εTerm l f) (εTerm l t) 
  εTerm l (TFix t)   = TFix (εTerm l t)
  εTerm l (TLam x t) = TLam x (εTerm l t)
\end{mcode}

\paragraph{Preservation of Noninterference}
The proof of noninterference is preserved, since, 
intuitively, erasure on the new terms is a homomorphism. 
%
The only extension is on the @simulationsTerm@
theorem where, in the cases of $\beta-$reduction 
(\ie when a $\lambda-$term is applied to the application or fix operator)
we need a theorem  
that erasure is a homomorphism on substitution:
\begin{mcode}
  homomorphicSubst 
    :: Label l 
    => l:l 
    -> x:Var 
    -> tx:Term 
    -> t:Term 
    -> {   εTerm l (subst x tx t) 
        == subst x (εTerm l tx) (εTerm l t)}
\end{mcode}


==> lio.tex <==
\section{Monadic Terms for the Label State}\label{sec:lio}

Next, we extend programs with effectful computations 
that depend on a label. 
\begin{mcode}
  data Program l 
    = PgHole 
    | Pg {pLabel :: l, pTerm :: Term l}
\end{mcode}
For the program @Pg lc t@, 
the label @lc@ indicates the current observation label
under which the term @t@ is executed. 
This current label tracks the label of all values in scope, similar 
to a program counter label. 

\paragraph{Terms}
We extend the terms with standard monadic expressions
and monadic expressions that manipulate the current label. 
The term @TGetLabel@ returns the current label. 
@TBind@ and @TReturn@ represent the standard monadic 
methods. 
@TLIO@ is the result of a monadic computation. 
%
Finally, we add the exception term @TException@
to represent the runtime error when a bind is performed 
on non-monadic terms.
\NV{Check with James about exceptions.} 
%
\begin{mcode}
  data Term l = ... 
    | TGetLabel 
    | TReturn (Term l)
    | TBind (Term l) (Term l) 
    | TLIO (Term l)
    | TException
\end{mcode}
%
\paragraph{Values}
We extend the values with the expressions that cannot get evaluated, 
that is, the monadic value @TLIO@ and exceptions. 
\begin{mcode}
  isValue :: Term l -> Bool 
  isValue (TLIO _)   = True 
  isValue TException = True 
  isValue _          = False 
\end{mcode}


\paragraph{Evaluation}
Next, we extend the evaluation function to account for monadic expressions.
\begin{mcode}
  eval :: Label l => Program l -> Program l
  eval (Pg lc (TReturn t))
    = Pg lc (TLIO t)
  eval (Pg lc TGetLabel)
    = Pg lc (TReturn (TLabel lc))
  eval (Pg lc (TBind t1 t2))
   | Pg lc' (TLIO t1') <- #evalStar (Pg lc t1)#
   = Pg lc' (TApp t2 t1')
   | otherwise 
   = Pg lc TException
\end{mcode}
The return expression returns the monadic value @LIO@. 
The get label expression returns the current label. 
To bind the expressions @t1@ and @t2@, first 
the expression @t1@ is fully evaluated into a monadic value; 
then the resulting value is applied to @t2@. 
If @t1@ is not evaluated into a monadic value, 
then evaluation returns an exception. 
%

The evaluation of the monadic bind uses % for full evaluation 
the function @evalStar@, the transitive closure of 
the evaluation function, for full evaluation. 
%
If @evalStar@ reaches a value term, then it returns. 
Otherwise, it recursively calls itself after one step of evaluation.  
\begin{mcode}
  evalStar :: Label l => Program l -> Program l
  evalStar PgHole
    = PgHole
  evalStar (Pg lc t) | isValue t 
    = (Pg lc t)
  evalStar p
    = #evalStar (eval p)#
\end{mcode}

\paragraph{Termination of evaluation function.}
Since programs might diverge, 
the evaluation function might too diverge. 
%
In fact, in the above mutually recursive definitions 
of @eval@ and @evalStar@ Liquid Haskell will fire 
a termination error in the underlined recursive calls. 

We restrict the definition of the evaluation relation to only 
accept terminating programs, where the termination predicate 
is axiomatized to encode properties of termination. 

We define a logical function that returns the evaluation steps 
of a terminating program: 
%
\begin{mcode}
  evalSteps :: Program l -> Nat
\end{mcode}
%
We then declare than the evaluation function 
on terminating programs terminates, 
since the @evalSteps@ of the input program is decreasing. 
%
\begin{mcode}
  eval     :: Label l => p:{Program l | terminates p}
           -> Program l
           /  [evalSteps p, 1]

  evalStar :: Label l => p:{Program l | terminates p}
           -> Program l
           /  [evalSteps p, 2]
\end{mcode}
Concretely, we use the termination metric annotation below 
to express that among the mutually recursive calls of
@eval@ and @evalStar@, the termination metrics 
@[evalSteps p, 1]@ and @[evalSteps p, 2]@ should respectively 
decrease. 
%
That is, calls where @evalSteps@ decreases are always allowed. 
But also, @evalStar@ can call @eval@ on inputs with unchanged 
@evalSteps@ (since @evalStar p@ calls @eval p@). 

Next, 
we axiomatize the relation between terminating programs 
and their evaluation steps. 
We assume that when a program terminates, its evaluation 
requires strictly less steps and also terminates.
%
\begin{mcode}
  assume evalStepsAxiom 
    :: Label l 
    => p:{Program l | terminates p }   
    -> { terminates (eval p) && 
         evalSteps (eval p) < evalSteps p } 
  evalStepsAxiom _ = ()
\end{mcode}

Also we assume that if a @TBind t1 t2@ terminates, 
then @t1@ terminates in fewer evaluation steps. % so does @t1@ needing less evaluation steps. 
\begin{mcode}
  assume bindAxiom 
    :: Label l 
    =>  lc:l  
    -> t1:Term l 
    -> t2:{Term l | terminates (Pg lc (TBind t1 t2))}
    ->  {terminates (Pg lc t1) && 
         evalSteps (Pg lc t1) < 
         evalSteps (Pg lc (TBind t1 t2))}
  bindAxiom _ _ _ _ _ = () 
\end{mcode}
%
We use these assumptions 
to remove the termination error in the evaluation definition. 
%
The standard library @const@ function is used to call these axioms while ignoring their result. 
%% To call these axioms, we use a cast function 
%% @cast _ x = x@ that merely returns its second 
%% argument, 
%% while putting the refinements of the first into the proving 
%% environment. 
%
The two mutually recursive calls are repaired as presented below:
%
\begin{mcode}
  | Pg lc' (TLIO t') <- evalStar (Pg l t1) `const` bindAxiom l t1 t2
  ... 

  evalStar p
    = evalStar (eval p) `const` evalStepsAxiom p
\end{mcode}

\paragraph{Erasure} 
We adjust program erasure to account for the current label.
\begin{mcode}
  ε :: Label l => l -> Program l -> Program l
  ε _ PgHole = PgHole
  ε l (Pg lc t) 
    | lc canFlowTo l
    = Pg lc (εTerm l t) 
    | otherwise 
    = PgHole  
\end{mcode}
To erase a program using label @l@, 
if the current label of the program can flow into @l@
then we just erase the term of the program, 
otherwise, we return a program hole.

We homomorphically extend term erasure definition 
on monadic terms.


\subsection{Noninterference}\label{subsection:lio:noninterference}
To prove nonintereference, we need to update the program simulations proof 
for 1) programs whose label cannot flow into the erasing label and 
2) programs with monadic terms. 

The case when the program label does not flow into
the erasing label is easy, since 
program erasure leads into a program hole
that evaluates into an identity.
\begin{mcode}
  simulations l (Pg lc t) 
    | not (lc canFlowTo l) 
    =   ε l (eval (ε l (Pg lc t)))
    ==. ε l (eval PgHole)
    ==. ε l PgHole
    ==. PgHole
    ==. ε l (Pg lc (evalTerm t))
    ==. ε l (eval (Pg lc t)) 
    *** QED
\end{mcode}

We extend the simulations proof for the case of the monadic operations. 
The get label and return cases are trivial and proceed by rewriting and idempotence. 

The interesting case is to prove that simulations are preserved in 
the case of the bind: 
\begin{mcode}
      ε l (eval (ε l (Pg lc cc m (TBind t1 t2)))) 
   ==. ...
   == ε l (eval (Pg lc cc m (TBind t1 t2)))
\end{mcode}

The evaluation of @TBind@ splits cases on whether or not 
@t1@ evaluates into a monadic value and then returns the label 
of the evaluated @t1@. 
Thus, our proof spits cases on 
the result of the evaluation of @t1@ and 
if the resulting label can flow into @l@. 

The interesting case appears 
when both @t1@ and its erasure evaluate into a
monadic value with labels that can flow into @l@.
Then, the proof proceeds by rewriting
until we reach a point where the
label and term resulted by the evaluation 
of @t1@ and each erasure needs to be equated: 
\begin{mcode}
  simulations l (Pg lc (TBind t1 t2))
    | Pg εlc' (TLIO εt') <- evalStar (Pg lc εt1)
    , Pg  lc' (TLIO t' ) <- evalStar (Pg lc t1)
    , εlc' canFlowTo l, lc' canFlowTo l =
        let εt1 = εTerm l t1 in
        let εt2 = εTerm l t2 in
        ε l (eval (ε l (Pg lc (TBind t1 t2))))
    ==. ε l (eval (Pg lc (εTerm l (TBind t1 t2))))
    ==. ε l (eval (Pg lc (TBind εt1 εt2)))
    ==. ε l (Pg εlc' (TApp (εTerm l t2) εt'))
    ==. Pg εlc' (εTerm l (TApp (εTerm l t2) εt'))
    ==. Pg εlc' (TApp (εTerm l εt2) (εTerm l εt'))
    ==. Pg εlc' (TApp εt2 (εTerm l εt'))
        ? εTermIdempotent l t2
    ==. Pg lc'  (TApp εt2 (εTerm l t'))
\end{mcode}

To prove the last equation, 
we make a subproof that equates the
label and term resulted by the evaluation 
of @t1@ with the corresponding erasure using the theory of data types:
\begin{mcode}
          ? (
          Pg lc' (TLIO (εTerm l t'))
      ==. Pg lc' (εTerm l (TLIO t')) 
      ==. ε l (Pg lc' (TLIO t'))
      ==. ε l (evalStar (Pg lc t1))
          ? bindAxiom lc t1 t2 
      ==. ε l (evalStar (ε l (Pg lc t1))) 
          ? simulationsStar l (eval p)  
      ==. ε l (evalStar (Pg lc (εTerm l t1)))
      ==. ε l (Pg εlc' (TLIO εt'))
      ==. Pg εlc' (εTerm l (TLIO εt'))
      ==. Pg εlc' (TLIO (εTerm l εt'))
      *** QED 
          )
\end{mcode}
For example, since @Pg lc' _ == Pg εlc' _@, 
then the solver concludes that @lc' == εlc'@. 
%
This subproof uses the simulation property of
@evalStar@ as discussed later, 
as well as the @bindAxiom@ to prove that the mutual recursive proof 
(between @simulations@ and @simulationsStar@) is terminating and thus well defined. 

After the intermediate label and expressions 
are equated, the proof simply concludes by rewriting. 
\begin{mcode}
    ==. Pg lc' (TApp εt2 (εTerm l t'))
    ==. Pg lc' (εTerm l (TApp t2 t'))  
    ==. ε l (Pg lc'(TApp t2 t'))  
    ==. ε l (eval (Pg lc (TBind t1 t2)))  
    *** QED 
\end{mcode}


The simulation theorem on @evalStar@
states the simulation property between 
@evalStar@ and @evalStar . ε l@.
\begin{mcode}
  simulationsStar 
    :: Label l 
    => l:l
    -> p:{Program l | terminates p } 
    -> { ε l (evalStar (ε l p)) = ε l (evalStar p) } 
\end{mcode}
Much like the definitions of @eval@ and @evalStar@, 
the proof @simulations@ and @simulationsStar@
are mutually recursive and rely on @evalStep@ 
for termination proving. 
%
Moreover the proof relies on monotonicity of labels during evaluation
\begin{mcode}
  monotonicEvalStar 
    :: Label l 
    => p:{Program l | isPg p }
    -> { pLabel p canFlowTo pLabel (evalStar p) } 
\end{mcode}


The other cases of the bind proof are easier. 
If none of the evaluations are monadic values (@TLIO@) then evaluation of bind 
throws an exception that is propagated via erasure. 
%
Since erasure preserves the structure of the terms 
and evaluation is structurally defined, 
we prove that it is impossible for exactly one 
to be a monadic value. 
%
If none of the evaluated labels flow to @l@, 
then both sides return a hole, 
while due to simulations on @evaluationStar@
the returned labels need to be the same. 
\JP{revisit this once we add exceptions}
 


==> non-interference.tex <==
\section{Noninterference}\label{sec:non-interference}

 
\NV{James said to clarify that it is noninterference is termination insensitive} 
In this section we use a simplistic program definition to 
prove non interference.  
%
Later we extend the programs to useful ones 
and show how the noninterference proof is preserved. 

\subsection{Programs \& Labels}
We initially define a @Program@ Haskell datatype
to be simply a hole that will get later extended to contain 
labels of type @l@. 
\begin{mcode}	
  data Program l = PgHole 
  deriving Eq 
\end{mcode}
%
Evaluation of a program just returns the same program.
% 
\begin{code}
  eval :: Program l -> Program l 
  eval PgHole = PgHole 
\end{code}
%
Labels are abstractly represented by the Haskell type class 
@Labels@. 
For now we just define the ordering method  @(canFlowTo)@
and in \S~\ref{sec:labels} we extend to the class to represent a lattice.  
%
\begin{mcode}	
  class Label l where 
    (canFlowTo) :: l -> l -> Bool 
\end{mcode}

\subsubsection{Erasure \& Noninterference}

We define the erase function @ε@
that erases all the sensitive data (classified above l)
of the program.
\begin{mcode}
  ε :: Label l => l -> Program l -> Program l 
  ε l PgHole = PgHole 
\end{mcode}

Noninterference states that for each observation label @l@
and two terminating programs @p1@ and @p2@, 
if the two programs are equal at observation level @l@
then their evaluation will also be equal as seen by an attacker 
at observation level @l@.
%
We express noninterference as the following refinement type
%
\begin{mcode}	
  nonInterference
   :: Label l 
   => l:l  
   -> p1:{Program l  | terminates p1} 
   -> p2:{Program l  | terminates p2}
   -> {ε l p1 == ε l p2}
   -> p1':{Program l | eval p1 == p1' } 
   -> p2':{Program l | eval p2 == p2' } 
   -> {ε l p1' == ε l p2'}  
\end{mcode}
\NV{Shouldn't this be evalStar? Now we only do one step of evaluation.}

For some refinement @p@ we write @{p}@
to express the unit Haskell type refined 
with @p@, \ie @{v:() | p}@.
%
That is, @nonInterference@ is a Haskell function 
that always returns a unit value
yet its type is refined to express the noninterference theorem. 
%
Later we define the body of @nonInterference@
to constitute a proof that the theorem holds. 

The predicate @terminates@
is a logical predicate (\ie not a Haskell function)
that axiomatized program termination 
and is later (\S~\ref{sec:lio}) used justify well formedness of our proof. 
%
We use Liquid Haskell's @measure@ token to define the termination 
logical predicate 
\begin{mcode}
  measure terminates :: Program l -> Bool
\end{mcode}


\subsection{Simulations}\label{subsec:non-interference:simulations}

To prove noninterference we use a simulations property
between program evaluation and the composition of 
erasure and program evaluation as depicted in Figure~\ref{fig:simulation}.
%
Intuitively, erasing sensitive data and applying @ε l . eval@
is the same as applying @eval@ and then erasing the sensitive data. 

\begin{figure}
\begin{tikzpicture}
  \matrix (m) [matrix of math nodes,row sep=3em,column sep=10em,minimum width=2em]
  {
    \texttt{p} & \texttt{p'} \\
     \epsilon \texttt{ l p} & \epsilon \texttt{ l p'} \\};
  \path[-stealth]
    (m-1-1) edge node [left] {$\epsilon \texttt{ l}$} (m-2-1)
            edge  node [below] {$\texttt{eval}$} (m-1-2)
    (m-2-1.east|-m-2-2) edge node [below] {$\epsilon \texttt{ l . eval}$} (m-2-2)
    (m-1-2) edge node [right] {$\epsilon \texttt{ l}$} (m-2-2);
\end{tikzpicture}
\caption{Simulation between $\texttt{eval}$ and $\epsilon\texttt{ l . eval}$.}
\label{fig:simulation}
\end{figure}

We express the simulations property using 
a refinement type that states that 
for each label @l@
and terminating program @p@
the simulations equality holds. 

\begin{mcode}
  simulations 
  :: Label l
  => l:l
  -> p:{Program l | terminates p} 
  -> {ε l (eval (ε l p)) = ε l (eval p)}
\end{mcode}  
   
Since erasure and evaluation are defined to be identities   
the proof of simulations is straightforward. 
%
The Haskell definition of @simulations@ 
is using Liquid Haskell's equational reasoning to 
simply equate the left and right hand side of the equality.
%   
\begin{mcode}
  simulations l PgHole 
    =   ε l (eval (ε l PgHole))
    ==. ε l (eval PgHole)
    *** QED 
\end{mcode}

The infix operator @(==.)@ returns its second argument 
while the ``postfix'' @*** QED@ casts its argument into a unit. 

\begin{mcode}
  (==.) :: a -> a -> a
  _ ==. x = x 

  data QED = QED
  
  (***) :: a -> QED -> ()  
  _ *** QED = ()
\end{mcode}
%
Using these operators the body of @simulations@
is defined to resemble a mathematical proof 
that equates @ε l (eval (ε l p))@
with @ε l (eval p)@
simply by unfolding the definition of @ε@ 
with inputs @l@ and @p@. 
%
Since Liquid Haskell by default checks that 
all the functions are terminating and defined for all 
inputs, @simulations@ is a total function
thus can soundly be seen as a mathematical proof. 


\subsection{Proof on Noninterference}

We prove noninterference 
by defining the body of the Haskell 
@nonInterference@
using equational reasoning 
and appropriately invoking the @simulations@ 
theorem.

\begin{mcode}
  nonInterference l p1 p2 equivProof p1' p2' 
    =   ε l p1'
    ==. ε l (eval p1)
    ==. ε l (eval (ε l p1)) ? simulations l p1 
    ==. ε l (eval (ε l p2)) ? equivProof
    ==. ε l (eval p2)       ? simulations l p2 
    ==. ε l p2' 
    *** QED 
\end{mcode}

The explanation operator @(?)@
is used to explain the equational steps 
by calling existing theorems. 
%
\begin{mcode}
  (?) :: a -> Proof -> a 
  x ? _ = x 
\end{mcode}


In the rest, we 
extend the programs definition with 
basic lambda terms (\S~\ref{sec:lambda}), 
label operations (\S~\ref{sec:labels}), 
basic monadic terms (\S~\ref{sec:lio})
and monadic terms that allow 
labeling values (\S~\ref{sec:labeling})
restriction of data access (\S~\ref{sec:clearance})
and data base operators (\S~\ref{sec:db}).
%
For each such extension 
we accordingly extend the definitions of 
program evaluation and erasure 
and prove that the simulations property, 
and thus noninterference, is preserved. 


==> tolabeled.tex <==
\section{Scoped Contexts} %Transferring Protection}
\label{sec:tolabeled}

With the monadic expressions introduced in~\S~\ref{sec:labeling}, 
programs can interact with labeled values. 
A consequence of these expressions is that the current label in 
the environment is monotonically increasing. 



\paragraph{Terms}
To limit the increase in current label, the term @TToLabeled tl t@ is introduced.
Term @t@ is a monadic computation whose result is labeled by the label @tl@. 
Once the monadic computation is complete, the current label is reset to its initial value. 
% 
% that can run with a current label 
% 
% 
% scope of ...
% 
\begin{mcode}
  data Term l = ... 
   | TToLabeled (Term l) (Term l)
\end{mcode}

\paragraph{Values}
@TToLabeled tl t@ is not a value.
\begin{mcode}
  isValue (TToLabeled _ _) = False  
\end{mcode}

\paragraph{Evaluation}
Term @t@ is fully evaluated to its monadic value. 
As long as its resulting current label does not exceed @l@ and the initial current label can flow to @l@, the value is labeled with @l@ and returned. 
In addition, the current label reverts to its initial value from before evaluating @t@. 
Otherwise, an exception is thrown. 

\JP{Do we need a const/cast axiom call here?}
\JP{I added TLIO. I think we need to update the proof to include fromTLIO as well.}
\begin{mcode}
  eval (Pg lc (TToLabeled (TLabel l) t))
    | Pg lc' (TLIO t') <- evalStar (Pg lc t)
    , lc  canFlowTo l, lc' canFlowTo l 
    = Pg lc (TReturn (TLabeled l t'))
    | otherwise 
    = Pg lc TException

  eval (Pg lc (TToLabeled tl t))
    = Pg lc (TToLabeled (evalTerm tl) t)
\end{mcode}

\paragraph{Erasure}
\JP{The original proof + Deian's paper eagerly erase here too.}
\begin{mcode}
  εTerm l (TToLabeled tl t)  
    = TToLabeled (εTerm l tl) (εTerm l t)
\end{mcode}

\paragraph{Noninterference}
The proof proceeds by case splitting 
and mutually recursively calling the simulations star theorem, 
similar to the bind proof of~\S~\ref{sec:lio}.








